RARES: Runtime Attack Resilient Embedded System Design Using Verified Proof-of-Execution

Modern society is getting accustomed to the Internet of Things (IoT) and Cyber-Physical Systems (CPS) for a variety of applications that involves security-critical user data and information transfers. In the lower end of the spectrum, these devices are resource-constrained with no attack protection. They become a soft target for malicious code modification attacks that steals and misuses device data in malicious activities. The resilient system requires continuous detection, prevention, and/or recovery and correct code execution (including in degraded mode). By end large, existing security primitives (e.g., secure-boot, Remote Attestation RA, Control Flow Attestation (CFA) and Data Flow Attestation (DFA)) focuses on detection and prevention, leaving the proof of code execution and recovery unanswered. To this end, the proposed work presents lightweight RARES -- Runtime Attack Resilient Embedded System design using verified Proof-of-Execution. It presents first custom hardware control register (Ctrl_register) based runtime memory modification attacks classification and detection technique. It further demonstrates the Proof Of Concept (POC) implementation of use-case-specific attacks prevention and onboard recovery techniques. The prototype implementation on Artix 7 Field Programmable Gate Array (FPGA) and state-of-the-art comparison demonstrates very low (2.3%) resource overhead and efficacy of the proposed solution.

==> background.tex <==
\section{Background and Related Work}
\par This section defines essential concepts used and referenced by the proposed framework, followed by exploring related state-of-the-art works.

\section{Security Model}
\subsection{\bf{Security Properties}} \label{securityprop}
\emph{SRACARE} has derived eight (A1-A8) security properties
escalation or interruption.
\subsection{\bf{Adversary and Threat Model}}\label{themo}
The adversary: 
\begin{itemize}
	\item{}has full control over the firmware and software of the device.
	\item{}can perform an unauthorized read or write to the flash memory.
	\item{}can modify existing code by re-arranging, flipping the bits, buffer-over-flow, or fault injection attacks. 
	\item{}cannot attack protected ROM.
\end{itemize}
\par The side-channel attack, physical access, damaging device, and control flow integrity attacks are out of scope for the proposed work.
\subsection{\bf{Design Choices}} \label{assum1}
\par \emph{SRACARE} system incorporates the following design choices to satisfy the security properties discussed in subsection~\S\ref{securityprop}.\\

==> care.tex <==
\section{SRACARE Framework}
%\vspace{-1em}
\subsection{\bf{System Design}} \label{SRACAREO}
\par  shows the top-level design overview of the \emph{SRACARE} framework, highlighted are two main security-enhancing techniques proposed by this work: 1) Lightweight, secure communication protocol and 2) Secure boot with \emph{CARE} and RA architecture for the P\textsubscript{r} device. 
\subsection{\bf{System Operation}} \label{working}
\par The working of \emph{SRACARE} system is divided into four main steps: 1) Secure Communication Protocol, 2) Secure Boot, 3) Resilience and Recovery, and 4) Remote Attestation. \\ 
{\bf{1) Secure Communication Protocol}:}\label{SCP} The communication starts by the V\textsubscript{r} sending nonce n1 to the P\textsubscript{r}. The P\textsubscript{r} computes Hmac(K, n1) using the crypto-core and generates n2 by performing Hmac(K, T).

==> conclusion.tex <==
\section{Conclusion}
\emph{SRACARE} demonstrates the POC framework that performs the run-time and boot-time integrity and authenticity checks, secure boot with onboard recovery, and remote attestation on the \mbox{RISC-V} based small embedded and IoT devices. It implements the novel lightweight,  secure authenticated communication protocol. It provides the tools for the detection, protection and recovery from malicious code modification attacks. The experimental results show good protection against malicious code modification attacks, with only 8\% execution time overhead and a tiny increase in resource footprint. 

==> evaluation.tex <==
\section{Evaluation} \label{Evaluation}
This section describes the chain-of-trust theory, resource utilization, and performance analysis for each submodule in \emph{SRACARE} framework design, and comparison with state-of-the-art solutions.  
\vspace{-.7em}
\subsection{\bf{Chain-of-Trust}}\label{chainoftrust}
The work presented in  defines the secure boot process as a chain of many small layers of the boot codes executed in a specific sequence. 

\subsection{\bf{Code Authentication (CA) Unit}}\label{PA}
%\vspace{-.1em}
\par The key component of the Code Authentication (CA) unit is crypto-core (HMAC-SHA256). To estimate the initial performance, power, and resource utilization, our evaluation setup uses both hardware and software implementation of
\subsection{\bf{Resilience Engine (RE)} }
\par The Resilience Engine (RE) is implemented in software for the POC work. 
\subsection{\bf{System Performance}}\vspace{-.5em}
\par For \emph{SRACARE} system {\bf{timing analysis}}, a test application of 5.6~KB is divided into six 1~KB chunks and the total time for the system boot-up with and without the proposed framework is calculated and presented in .

\subsection{\bf{Resource Utilization}}
Inspired from the googles opentitan, the prototype implementation uses the Ibex \mbox{RISC-V} core for the RTL design.
%\vspace{-1em}
\subsubsection{\bf{Hardware Resource Utilization on FPGA}}

\subsubsection{\bf{Software Resource Utilization}} 
The POC work has implemented the RE sub-module and secure communication protocol in software. It requires 61 additional lines of (C language) code for RE (which includes cycle calculation and analysis code for Ibex) and 5~KB of extended ROM storage.It requires 108 additional lines of code (C language) on the P\textsubscript{r} side for secure RA (UART) protocol and novel n2 generation logic implementation. \emph{SRACARE} increases the total software code base by 10\%.
%%\vspace{-1em}
\subsection{\bf{Comparison with the State-of-the-art Solutions}}
%%\vspace{1em}
\par Since \mbox{RISC-V} is a relatively new architecture, authors of this work did not found any {\bf{secure boot with resilience or recovery}} implementation for state-of-the-art comparison.\\

\subsubsection{\bf{Qualitative Comparison}} 
%\vspace{-1em}
\subsubsection{\bf{Quantitative Comparison}}\label{quantify}
%\vspace{-1em}
%\par Table~\ref{care1} enumerates the quantitative comparison of the complete \emph{SRACARE} system,


